Averaging Essential and Fundamental Matrices in Collinear Camera Settings

Global methods to Structure from Motion have gained popularity in recent years. A significant drawback of global methods is their sensitivity to collinear camera settings. In this paper, we introduce an analysis and algorithms for averaging bifocal tensors (essential or fundamental matrices) when either subsets or all of the camera centers are collinear. We provide a complete spectral characterization of bifocal tensors in collinear scenarios and further propose two averaging algorithms. The first algorithm uses rank constrained minimization to recover camera matrices in fully collinear settings. The second algorithm enriches the set of possibly mixed collinear and non-collinear cameras with additional, "virtual cameras," which are placed in general position, enabling the application of existing averaging methods to the enriched set of bifocal tensors. Our algorithms are shown to achieve state of the art results on various benchmarks that include autonomous car datasets and unordered image collections in both calibrated and unclibrated settings.

==> Table_Kitti_Eucl.tex <==




==> Tables2.tex <==

\begin{table*}[tbh] \label{table:translation}
\tiny

\resizebox{\linewidth}{!}{%
\
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
&\multicolumn{3}{|c|}{ \textbf{ Our Method } }&\multicolumn{3}{|c|}{ \textbf{ }\cite{kasten2019algebraic} }  &    \multicolumn{3}{|c|}{ \textbf{LUD} \cite{ozyesil2015robust}} &\multicolumn{3}{|c|}{ \textbf{ 1DSFM }\cite{wilson2014robust} }  \\\hline
Data set & T_{R+T} & $T_{BA}$ & $T_{Tot}$ & T_{R+T} & $T_{BA}$ & $T_{Tot}$ &T_{R+T} & $T_{BA}$ & $T_{Tot}$ & T_{R+T} & $T_{BA}$ & $T_{Tot}$  \\\hline
Vienna Cathedral & {145} & 262 & {930}& {68} & 293 & {566} & 787 & 208 & 1467 & 323 & 3611 & 3934  \\\hline
Piazza del Popolo & {54} &39 & {143} & {26} & 27 & {87} & 88 & 31 & 162 & 42 & 213 &  255\\\hline
NYC Library & {55} & 80 & 214& {28} & 58 & 125 & 102 & 47 & 200 & 47 & 382 & 429 \\\hline
Alamo & {96} & 115& {509}&{47} & 155 & {327} & 385 & 133 & 750 & 152 &  646 &  798 \\\hline

Yorkminster & {67} & 100 &  296 & {33} & 116 & 207 & 103 & 148 & 297 & 71 & 955 & 1026  \\\hline
Montreal ND & {80} & 216 & 626& {41} & 170 & 494 & 271 & 167 & 553 & 93 & 1043  &  1136 \\\hline
Tower of London & { 89} & 132 & 280&{41} & 120 & 241 & 88 & 86 & 228 & 61 & 750 & 811 \\\hline
Ellis Island & {40} & 44 & 170& {21} & 53 & 140 & - & - & - & 29 & 276 &  305  \\\hline
Notre Dame & {100} & 419 & {1070} & {52} & 277 & {720}& 707 & 126 & 1047 & 205 & 2139 &  2344  \\\hline
\end{tabular}
}
\caption {\small Running time in seconds for results in Table \ref{table:translation}. $T_{R+T}$ denote the time for motion averaging (for other methods rotation and translation estimation). $T_{BA}$ the time for bundle adjustment and $T_{Tot}$ is the total running time of the method, including the additional time for building the triangle cover. Empty cells represent image collections not tested by the authors.}\label{table:Times}
\end{table*}

\begin{table*}[tbh]
\tiny

\resizebox{\linewidth}{!}{%

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
 & &\multicolumn{5}{|c|}{ \textbf{Our Method } }&\multicolumn{5}{|c|}{ \textbf{ \cite{kasten2019algebraic} } } &    \multicolumn{5}{|c|}{ \textbf{LUD} \cite{ozyesil2015robust}} &\multicolumn{4}{|c|}{ \textbf{ 1DSFM }\cite{wilson2014robust} }  \\\hline
Data set & $N_c$ &$\bar{x}$ & $\tilde{x}$ &$\bar{x}_{BA}$ & $\tilde{x}_{BA}$ & $N_r$ & $\bar{x}$ & $\tilde{x}$ &$\bar{x}_{BA}$ & $\tilde{x}_{BA}$ & $N_r$ & $\bar{x}$ & $\tilde{x}$ &$\bar{x}_{BA}$ & $\tilde{x}_{BA}$ & $N_r$  & $\tilde{x}$ &$\bar{x}_{BA}$ & $\tilde{x}_{BA}$ & $N_r$ \\\hline
Vienna Cathedral & 836&{14.9} &4.9
&  {11.1
} & 2.0
 & 715 & {9.6} & 4.2 & 5.4 & 1.2  & 674 & 10 & 5.4 & 10 & 4.4 & 750  & 6.6 & 2e4 & {0.5} & 757  
\\\hline
Piazza del Popolo & 328& 6.7&3.1
 & 3.2
 & 0.8
 & 280 & 7.2 &  3.5 & {2.5} & {0.8} & 275 & {5} & {1.5} & 4 & 1.0 & 305  & 3.1 & 200 &2.6  & 303  

\\\hline
NYC Library & 332& 4.2 &2.7
  & 2.3
 & 0.8
 
& 281 & {3.3} &  2.2 & {1.1} & 0.47 & 277 & 6 & {2.0} & 7 & 1.4 & 320  & 2.5 & 20 & {0.4} & 292 

\\\hline
Alamo & 577& 2.6&1.1
 & 1.4
 & 0.3
 & 502 & 2.5  & 1.2  & {0.8} & 0.35 & 482 & {2} & {0.4} & 2 & {0.3} & 547 & 1.1 & 2e7 & {0.3} & 521  

 \\\hline

Yorkminster & 437&11.6& 3.1
 & 9.4
 & 1.0
 & 367 & 5.6 & {2.7}  & {1.9} & 0.8 & 341 & {5} & {2.7} & 4 & 1.3 & 404  & 3.4 &  500&{0.2}  & 395 
 
 \\\hline
Montreal ND & 450&2.0 &1  &1.2
 & {0.7
} & 433 & 1.9 &  1.0 & {0.6} & {0.4} & 416 & {1} & {0.5} & 1 & {0.4} & 435  & 2.5 &  1 & 0.9 & 425 
\\\hline
Tower of London & 572& 11.2 &4.6
 & 6.9
 & 1.4
 & 422 & {11.6} & 5.0 & {4} & 1.0 & 414 & 20 & {4.7} & 10 & 3.3 & 425 & 11 &   40&{0.4}  & 414 
 
\\\hline
Ellis Island & 227& 11.0&5.3
 & {4.4
} & 1.8
 & 214 & 14.1 & 6.1 & 5.3 & 1.7 & 211 & - & - & - & - & -  & 3.7 & 40 & {0.4} & 213 

 \\\hline
Notre Dame & 553& {1.7}&0.7 & 0.5
 & {0.2} & 536 & 1.8 & 0.8 & {0.4} & {0.2} & 529 & {0.8} & {0.3} & {0.7} & {0.2} & 536  & 10 & 7&  2.1 & 500  

\\\hline
\end{tabular}
}
\caption{\small Camera positions error in meters evaluated on the data sets of \cite{wilson2014robust}. \ag{this table might change a bit}}
\label{table:translation1dsfm}
\end{table*}


\begin{table}[tbh]


\caption{\small Mean position error calibrated setting, KITTI }\label{table:Kitti_Euc}\\
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c|c|c|c||c|c|c|c|c||c|c|c|c|c|}\hline
\multirow{2}{1.1em}{\textbf{DS}} & \multicolumn{5}{|c||}{ \textbf{5 Cameras}}& \multicolumn{5}{|c||}{ \textbf{10 Cameras}}& \multicolumn{5}{|c|}{\textbf{20 Cameras}} \\\cline{2-16}
& VP &  R4 &  \cite{kasten2019algebraic} &  \cite{ozyesil2015robust} &\cite{wilson2014robust}& VP & R4 & \cite{kasten2019algebraic} &  \cite{ozyesil2015robust} &\cite{wilson2014robust} & VP & R4 &  \cite{kasten2019algebraic} &  \cite{ozyesil2015robust} &\cite{wilson2014robust} \\\hline
 00 
 & \textbf{0.02}


 & {0.06
}
 & {0.36
}

 & 0.05
 &299.50


 & \textbf{0.04
}

 &{ 0.10
}

 & {1.34
}
 & 0.08

&0.94

 & {0.13
}

 & {0.35
}

 & {2.69
}

 & \textbf{0.11}

 &1.89

 \\\hline
 01 
 & \textbf{0.73
}

 & 1.41

 & {2.36
}

 & 1.16

&1.88

 & \textbf{1.09
}

 & 3.22


 & {5.47
}
 & 1.86

 &4.26

 & {3.57
}

 &5.21


 & {11.97
}

 & \textbf{2.57}

&5.87

\\\hline
 02 
 & \textbf{0.03
}

 & {0.04
}
 & 0.65


 & 0.11
&0.89

 & \textbf{0.09}


 & {0.12
}

 & {1.89
}
 & 0.13

&1.68

 & 0.34


 & \textbf{0.20
}

 & {4.20
}

 & 0.29

 &1.97

\\\hline
 03 
 & \textbf{0.07
}

 & {0.23
}
 & 0.28


 & 0.09

&0.55

 & {0.27
}

 & {0.41
}

 & 0.64

 & \textbf{0.08}

&0.97

 & {0.45
}

 & 1.52


 & 2.33

 & \textbf{0.12
}
 &1.83

\\\hline
 04 
 & \textbf{0.09
}

 & 0.26

 & 0.90


 & 0.18

&0.84
 & \textbf{0.07}

 & 0.34


 & 2.65

 & 0.18
 &1.74

 & \textbf{0.15
}

 & 0.60


 & {6.22
}

 & 0.39

 &4.21

\\\hline
 05 
 & \textbf{0.02
}

 & {0.06
}
 & 0.49


 & 0.07
&1166.56
 & \textbf{0.03}

 & {0.10
}

 & {1.37
}
 & 0.13

&30.14

 & \textbf{0.09
}

 & 0.24


 & {3.24
}

 & 0.19

 &2.02

\\\hline
 06 
 & \textbf{0.03
}

 & {0.16
}
 & {0.94
}

 & 0.14

 &1.37

 & \textbf{0.10
}

 & 0.28


 & {2.43
}
 & 0.17

&1.52

 & {\textbf{0.21}
}

 & 0.76

 & {5.73
}

 & {0.39
}
 &3.89

\\\hline
 07 
 & \textbf{0.02
}

 & 0.08

 & {0.30
}

 & 0.05
&7.95
 & {0.04
}

 & {0.18
}

 & 0.80

 & 0.06

&442.08

 & \textbf{0.09
}

 & 0.34


 & {1.74
}

 & {0.10
}
 &1.79
\\\hline
 08 
 & \textbf{0.02
}
 & {0.04
}
 & {0.40
}

 & 0.06

&0.62

 & \textbf{0.04}

 & \textbf{0.16
}

 & 0.92

 & 0.07

&49.13

 & \textbf{0.11
}

 & 0.25


 & {2.37
}

 & 0.15
 &2.33

\\\hline
 09 
 & \textbf{0.02}

 & {0.15
}
 & {0.62
}

 & 0.12

&21.07

 & {\textbf{0.06
}}

 & {0.24
}

 & 1.96

 & 0.10

 &0.96

 & 0.18


 & 0.53


 & {3.93
}

 & \textbf{0.14
}
 &2.97

\\\hline
 10 
 & \textbf{0.02}

 & {0.04
}
 & 0.61


 & 0.07

& 0.86

 & \textbf{0.05
}

 & 0.14


 & {1.65
}
 & 0.11

&1.42

 & \textbf{0.15}


 & 0.28


 & {3.01
}

 &  {0.17
} &2.54
\\\hline
\end{tabular}
}
\end{table}



\begin{table}[tbh]


\caption{\small Mean reprojection error  in pixels for non-calibrated setting, KITTI. The results are averaged per dataset.}\label{table:Kitti_Proj}\\
\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c|c|c||c|c|c|c||c|c|c|c|}\hline
\multirow{2}{1.em}{\textbf{}} & \multicolumn{4}{|c||}{ \textbf{5 Cameras}}& \multicolumn{4}{|c||}{ \textbf{10 Cameras}}& \multicolumn{4}{|c|}{\textbf{20 Cameras}} \\\cline{2-13}
& VP &  R4 &  \cite{kasten2018gpsfm} &  \cite{magerand2017practical} & VP & R4 &  \cite{kasten2018gpsfm} &  \cite{magerand2017practical} & VP & R4 &  \cite{kasten2018gpsfm} &  \cite{magerand2017practical} \\\hline
 00 
 & \textbf{0.12
}


 & \textbf{0.12}

 & {0.40
}

 & 0.13


 & \textbf{0.15}


 & \textbf{0.15}


 & 4.63 & {0.16
}



 &\textbf{ 0.16
}

 &\textbf{ 0.16}


 & {8.71
}

 & 0.18

 \\\hline
 01 
 & 0.90


 & {0.85
} & {2.43
}

 &\textbf{ 0.22}


 & 6.09


 & 1.49


 & 7.09& \textbf{0.32
}
 

 & 5.84


 & 6.77


 & {16.45
}

 &\textbf{ 0.41}

\\\hline
 02 
 & \textbf{0.12
}

 & \textbf{0.12}
 & 2.84


 & 0.13


 & \textbf{0.15}


 &\textbf{ 0.15}


 & 7.58& {0.16
}
 


 & \textbf{0.16}


 & \textbf{0.16}


 & {14.20
}

 & 0.19

\\\hline
 03 
 & \textbf{0.14
}

 & \textbf{0.14}

 & 0.91


 & 0.15


 & \textbf{0.17
}

 & \textbf{0.17}


 & 0.84 & 0.21




 & \textbf{0.19
}

 & 0.21


 & 4.60


 & 0.31
\\\hline
 04 
 & \textbf{0.12
}

 &\textbf{ 0.12}

 & 0.69


 & 0.14


 & \textbf{0.15
}

 & \textbf{0.15}


& 11.68 & 0.18

 


 & \textbf{0.18}


 & \textbf{0.18}


 & {39.80
}

 & 0.22
\\\hline
 05 
 & \textbf{0.13
}

 & \textbf{0.13}

 & 1.72

 & 0.15


 &\textbf{ 0.16}


 & \textbf{0.16}

& 9.89 & {0.19
}
 


 &\textbf{ 0.18}

 & \textbf{0.18}


 & {20.61
}

 & 0.27

\\\hline
 06 
 & \textbf{0.12}


 & \textbf{0.12}

 & {1.92
}

 & 0.13


 &\textbf{ 0.15}


 & \textbf{0.15}

 & 18.74& {0.17
}
 


 & \textbf{0.17}


 &\textbf{ 0.17}


 & {42.83
}

 & 0.21
\\\hline
 07 
 & 0.84


 & \textbf{0.16}

 & {1.02
}

 & \textbf{0.16}


 & \textbf{0.18
}

 & 0.23


& 3.80 & 0.22

 


 & \textbf{0.21}


 & 3.15


 & {11.28
}

 & 0.37

\\\hline
 08 
 & \textbf{0.13
}
 & \textbf{0.13
}
 & 0.90

 & 0.14


 & \textbf{0.16
}

 & 0.18


 & 4.16& 0.18

 


 & \textbf{0.18}


 & 0.21


 & {9.42
}

 & 0.22

\\\hline
 09 
 & \textbf{0.12
}

 & \textbf{0.12}
 & {1.44
}

 & 0.13


 & \textbf{0.14
}

 & \textbf{0.14}


 & 8.78& 0.16

 

 &\textbf{ 0.16}


 & \textbf{0.16}


 & {12.62
}

 & 0.19
\\\hline
 10 
 & \textbf{0.12
}

 & \textbf{0.12}

 & 1.91


 & 0.13

 & \textbf{0.15}


 & \textbf{0.15}


 & 4.55& {0.17
}
 


 &\textbf{ 0.17
}

 & 0.20


 & {10.51
}

 &  0.20

\\\hline
\end{tabular}
}
\end{table}




